Neo: A Learned Query Optimizer

Query optimization is one of the most challenging problems in database systems. Despite the progress made over the past decades, query optimizers remain extremely complex components that require a great deal of hand-tuning for specific workloads and datasets. Motivated by this shortcoming and inspired by recent advances in applying machine learning to data management challenges, we introduce Neo (Neural Optimizer), a novel learning-based query optimizer that relies on deep neural networks to generate query executions plans. Neo bootstraps its query optimization model from existing optimizers and continues to learn from incoming queries, building upon its successes and learning from its failures. Furthermore, Neo naturally adapts to underlying data patterns and is robust to estimation errors. Experimental results demonstrate that Neo, even when bootstrapped from a simple optimizer like PostgreSQL, can learn a model that offers similar performance to state-of-the-art commercial optimizers, and in some cases even surpass them.

==> apx_q_learning.tex <==
\section{Q Learning}
\label{apx:q}
Here, we explain the strong connection between \system's value network and Q learning~\cite{q}, a traditional reinforcement learning technique. We first provide a brief summary of Q learning. Readers unfamiliar with Q learning may wish to see~\cite{rl_book} for an introduction. Note that, in the main text of the paper, we refer to minimizing latency, but here we will refer to maximizing reward in order to match the notation used in the reinforcement learning community (one can think of the reward as the negative latency). 

In a traditional reinforcement learning context, an agent at time $t$ observes a state $s_t$ and selects an action $a_t$, which results in the agent receiving some reward $r_t$ and being placed into a new state $s_{t+1}$. The goal is to find the series of actions that yields the greatest sum of rewards. Q learning~\cite{q, dqn} solves this problem by building a $Q$ function which makes a state/action pair to a value. When the agent observes state $s_t$, the agent selects the action with the highest Q value.

This Q function is updated after each intermediate reward $r_t$ is received, such that:

\begin{equation*}
Q^\prime(s_t, a_t) = (1 - \alpha) Q(s_t, a_t) + \alpha\left(r_t + \gamma \times \max_a Q(s_{t+1}, a)\right)
\end{equation*}

\noindent where $0 < \alpha \leq 1$ is the learning rate (the rate at which new information trumps older information) and $0 \leq \gamma \leq 1$ is the discount factor (how much to value short-term rewards vs. long-term rewards).

In the context of query optimization, there are no short-term rewards at all (a reward can only be determined after the query is executed, i.e. after the last action), so the only reasonable value of $\gamma$ is 1 (a value lower than 1 would indicate a preference for non-existent short-term rewards). Further, for all actions except the final action, $r_t$ is zero, and for the final action, the $\max$ term is zero, as no further actions can be taken. In fully deterministic environments, an $\alpha$ value of 1 is optimal~\cite{rl_book}. Therefore, for query optimization, we can rewrite the Q learning update rule as:

\begin{equation*}
Q^\prime(s_t, a_t) =
  \begin{cases}
     r_t & \mbox {$s_t$ is a final} \\
    \max_a Q(s_{t+1}, a) & \mbox{otherwise}
  \end{cases}
\end{equation*}

Intuitively, the rewritten Q function says that, for actions that result in a complete execution plan, return the final reward. Otherwise, return the reward achieved by playing the action currently believed to be best (the action that maximizes $Q$). This is precisely the function that we train the \system value network to learn. While this training will only result in an approximation of the $Q$ function (similar to other deep reinforcement learning techniques~\cite{dqn}), and will bypass the iterative updating procedure used in Q learning, there is still a strong connection between the two techniques.

It is worth noting that setting the learning rate, $\alpha$, to 1 has been shown to be optimal if the exact values of the Q function are being tracked: i.e., stored in a table, and not approximated by a neural network. To the best of our knowledge, there are no formal proofs indicating the optimality of any particular learning rate when the Q function is approximated by a neural network.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> challenges.tex <==
\section{Challenges - MOHAMMAD}
Goal of this section: motivate the complexity of the learn-from-demo + tree conv + search technique.

Cold start problem: randomly sampled query plans are catastrophic~\cite{howgood}. Two fundamental reasons this justifies divergence from standard DRL: (1) in normal DRL, getting the reward does not depend on the how good you are, e.g. if you suck at PacMan getting the score takes just as long as if you are good at PacMan (just read the number), but, if you are bad at query optimization, then getting the ``score'' requires executing a plan that could take months. (2) intuitively, you can learn much faster with an expert demonstrating something than you can on your own (ex: babies acquiring language), and we want our algo to be data efficient.

Unique state structure: for DQN on Atari, input is an image, so we use conv. But for us, the input is a tree structure. Tree conv is thus an intuitive inductive bias~\cite{inductive_bias_rl} to apply, because intuitively we can find patterns that look a lot like filters: joining table A and B with this predicate is bad, but joining table B and C is good.

Search technique: while DB folks have been using a heuristic + search (e.g. cost model + dynamic programming) for a long time, it is a relatively new innovation in RL world e.g. AlphaGo. By adding a search component, we decrease the impact of isolated bad predictions.

%Unlike prior work~\cite{rejoin, sanjay_wat}, our algorithm is not an off-the-shelf reinforcement learning scheme.

%\sparagraph{Why a new algorithm?} Previous work applying deep learning to query optimization have used reinforcement learning algorithms like proximal policy optimization (PPO)~\cite{ppo, rejoin} or deep Q learning (DQN)~\cite{sanjay_wat, dqn}. Both of these techniques have exhibited excellent performance on a wide variety of tasks in which the search space is very large and the underlying problem is stochastic (e.g., one does not know with absolute certainty the result of a particular action). While the search space in query optimization is certainly large, it is fundamentally \emph{deterministic}: choosing to join two relations together will always result in those two relations being joined together. Both DQN and PPO work in deterministic environments, but they are sample inefficient, i.e. they require substantially more training to learn a good policy.


%Deep reinforcement learning algorithms designed for deterministic environments, such as AlphaGo~\cite{alphago} and its many variants, assume an underlying environment that is competitive: the computer is playing against an adversarial opponent, constantly seeking to thwart their plans. Because of this, AlphaGo uses a combination of a neural network (which predicts the likelihood of victory in a state) and Monte Carlo Tree Search (a costly search technique proven to root out decisions beneficial to an adversary). However, query optimization is fundamentally \emph{non-adversarial} -- no one is trying to make a query's latency higher.\footnote{Excluding pay-by-the-hour cloud providers.}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> pari_jointree_example.tex <==
\begin{figure*}[t!]
    \begin{subfigure}[t]{0.5\textwidth}
    %{0.5\textwidth}
     %   \centering
        
\begin{tikzpicture}
\tikzset{edge from parent/.append style={very thick}}
\tikzset{every tree node/.style={draw,rectangle,fill=blue!20}}
\tikzset{level distance=30pt}
\tikzset{sibling distance=10pt}

\Tree 
[.LoopJoin
[.HashJoin 
    [.HashJoin 
        [.HashJoin 
            [.movie\_keyword ][.keyword ] 
        ]
        [.movie\_info 
        ]
    ] 
    [.title 
    ]
]
[.info\_type
 ]
]
\end{tikzpicture}
\caption{Joins Selected by Postgres for query in \ref{sql_query}}
    
    \end{subfigure}%
    ~ 
    \hspace{50pt}
    \begin{subfigure}[t]{0.5\textwidth}
  %      \centering

\begin{tikzpicture}
\tikzset{edge from parent/.append style={very thick}}
\tikzset{every tree node/.style={draw,rectangle,fill=blue!20}}
\tikzset{level distance=30pt}
\tikzset{sibling distance=10pt}

\Tree 
[.LoopJoin
[.LoopJoin 
    [.LoopJoin 
        [.LoopJoin 
            [.movie\_keyword ][.keyword ] 
        ]
        [.movie\_info 
        ]
    ] 
    [.title 
    ]
]
[.info\_type
 ]
]
\end{tikzpicture}
\caption{Joins Selected by Postgres for query in \ref{sql_query}}
     
    \end{subfigure}
    \caption{Caption place holder}
\end{figure*}
